MambAttention: Mamba with Multi-Head Attention for Generalizable Single-Channel Speech Enhancement

With new sequence models like Mamba and xLSTM, several studies have shown that these models match or outperform the state-of-the-art in single-channel speech enhancement and audio representation learning. However, prior research has demonstrated that sequence models like LSTM and Mamba tend to overfit to the training set. To address this, previous works have shown that adding self-attention to LSTMs substantially improves generalization performance for single-channel speech enhancement. Nevertheless, neither the concept of hybrid Mamba and time-frequency attention models nor their generalization performance have been explored for speech enhancement. In this paper, we propose a novel hybrid architecture, MambAttention, which combines Mamba and shared time- and frequency-multi-head attention modules for generalizable single-channel speech enhancement. To train our model, we introduce VB-DemandEx, a dataset inspired by VoiceBank+Demand but with more challenging noise types and lower signal-to-noise ratios. Trained on VB-DemandEx, MambAttention significantly outperforms existing state-of-the-art discriminative LSTM-, xLSTM-, Mamba-, and Conformer-based systems of similar complexity across all reported metrics on two out-of-domain datasets: DNS 2020 without reverberation and EARS-WHAM_v2. MambAttention also matches or outperforms generative diffusion models in generalization performance while being competitive with language model baselines. Ablation studies highlight the importance of weight sharing between time- and frequency-multi-head attention modules for generalization performance. Finally, we explore integrating the shared time- and frequency-multi-head attention modules with LSTM and xLSTM, which yields a notable performance improvement on the out-of-domain datasets. Yet, MambAttention remains superior for cross-corpus generalization across all reported evaluation metrics.

==> Text/01Introduction.tex <==
\section{INTRODUCTION}
\IEEEPARstart{S}{peech} enhancement aims to improve the speech intelligibility and speech quality of noisy speech signals, by removing background noise and recovering the desired speech signal. It is a widely studied subject, since speech enhancement is both challenging and has a wide array of applications such as hearing assistive devices, mobile communication devices, speech recognition systems, and speaker verification systems. 

Over the last decade, research on the single-microphone setting, also known as single-channel speech enhancement, has developed from using classical signal-processing techniques such as Kalman filtering \cite{paliwal1987speech}, subspace approaches \cite{ephraim1995signal}, and Minimum Mean Square Error Short-Time Spectral Amplitude estimation \cite{ephraim1984speech, griffin1984signal, ephraim1985speech} to using deep neural networks (DNNs) \cite{xu2014regression, kolbaek2016speech}. As the field of deep learning evolves, new neural architectures emerge. This has led to a large selection of deep learning-based single-channel speech enhancement systems using a variety of neural architectures such as deep denoising autoencoders \cite{lu2013speech}, recurrent neural networks (RNNs) and Long Short-Term Memory (LSTMs) networks \cite{weninger2014discriminatively, tesch22_interspeech}, convolutional neural networks (CNNs) \cite{fu2016snr,pandey2019new,kolbaek2020loss}, diffusion models \cite{lu2022conditional, richter2023speech, richter2024causal, gonzalez2024investigating}, generative adversarial networks (GANs) \cite{michelsanti17_interspeech, pascual17_interspeech, fu2019metricgan, fu2021metricgan+, abdulatif2024cmgan}, and state-space models (SSMs) \cite{sun2024dual,ku23_interspeech,du2024spiking}. With the advent of the Transformer \cite{vaswani2017attention}, attention-based speech enhancement systems have dominated the field, achieving state-of-the-art on several datasets \cite{mp-senet, lu2023explicit}.

However, scaled dot-product attention-based models like Transformers and Conformers \cite{gulati20_interspeech} scale poorly with sequence length and require large training datasets \cite{deoliveira22_interspeech, gong21b_interspeech}. Hence, recent works have focused on newly proposed sequence models with linear scalability with respect to sequence length such as Mamba \cite{gu2024mamba} and Extended Long Short-Term Memory (xLSTM) \cite{xlstm}. Mamba and xLSTM have already shown great promise in natural language processing (NLP) \cite{gu2024mamba, xlstm}, computer vision \cite{vim, visionxlstm}, and self-supervised audio representation learning \cite{audiomamba, audioxlstm}. Additionally, Mamba and xLSTM have recently been shown to match or outperform state-of-the-art speech enhancement systems \cite{semamba, xlstm-senet}. On the other hand, \cite{xlstm-senet} also found that a correctly configured LSTM-based model can actually match Conformer-, Mamba-, and xLSTM-based systems on the VoiceBank+Demand dataset \cite{voicebank, demand}. However, most papers reporting state-of-the-art often only evaluate in-domain speech enhancement performance. Arguably, in-domain speech enhancement performance may not be representative of performance in real-world environments, where speech and noise signals may vary significantly from the training data. For this reason, we focus on developing a speech enhancement algorithm that yields superior cross-corpus generalization performance. 

Prior works found that LSTMs overfit to the training dataset for automatic speech recognition in recurrent neural network transducers (RNN-T), which results in poor generalization performance \cite{chiu2021rnn,kim22f_interspeech}. To remedy this, \cite{chiu2021rnn} combines multiple regularization techniques during training, and uses dynamic overlapping inference by segmenting long utterances into multiple fixed-length segments, which are decoded independently. 
On the other hand, \cite{kim22f_interspeech} proposes using sparse self-attention layers in the Conformer RNN-T. Additionally, they hypothesize that during inference on long utterances, unseen linguistic context can accumulate excessively in the hidden state of the LSTM. They found that resetting the hidden states at silent segments can help mitigate this. Similarly, \cite{long2024dgmamba} hypothesizes that domain-specific information can potentially be
accumulated or even amplified in hidden states during propagation in the Mamba architecture, thus resulting in worse generalization performance. To mitigate this, they propose hidden state suppressing, which reduces the gap between hidden states across domains, and find  that this improves generalization performance in image recognition \cite{long2024dgmamba}.

Instead of focusing on the generalization performance of specific neural architectures, other works focus on the datasets themselves. In \cite{pandey2020cross}, it was established that poor generalization performance of speech enhancement DNNs stems from different recording conditions between datasets. It is revealed that the content of a corpus is more important than its size for speech enhancement generalization performance. Finally, it is shown that simply using a smaller frame shift in the short-time Fourier transform (STFT) significantly improves generalization performance. In \cite{gonzalez2023assessing}, a generalization assessment framework is presented. The framework accounts for the potential change in the difficulty of the speech enhancement task across datasets. Using this framework, it was found that for a feed-forward neural network (FFNN), two CNNs and an attention-based model, performance degrades the most in speech mismatches. Notably, it was revealed that while the most recent models displayed the best in-domain speech enhancement performance, their out-of-domain speech enhancement performance was beaten by the FFNN-based system \cite{gonzalez2023assessing}.
% In our paper, we augment Mamba with time- and frequency-multi-head attention blocks for generalizable single-channel speech enhancement.

Combining Mamba blocks with Transformer or attention blocks has already shown great promise in NLP \cite{lenz2025jamba, rensamba}, where the proposed models match or outperform state-of-the-art models on multiple benchmarks. However, the large token contexts used in NLP prevent the use of self-attention and Multi-Head Attention (MHA). Similarly, combining a Transformer encoder with an SSM results in state-of-the-art performance in automatic speech recognition (ASR)\cite{fathullah23_interspeech}. \Change{Beyond NLP and ASR, a hybrid Mamba and MHA model DeFT-Mamba \cite{deftmamba} was recently proposed for universal audio separation in multichannel polyphonic scenarios. By combining a gated convolution block (GCB) with a hybrid Mamba and MHA block across frequency- and time-dimensions to capture local frequency-time relations and position-wise global relations, DeFT-Mamba demonstrates state-of-the-art performance in multichannel separation.} In \cite{sui2024tramba}, Transformer and Mamba layers were combined in a U-Net architecture called TRAMBA. TRAMBA outperforms existing models in practical speech super resolution and enhancement on mobile and wearable platforms in a self-supervised setting. Finally, \cite{pandey2020cross} showed that augmenting an RNN with a self-attention block and a feedforward block substantially improves speech enhancement performance on out-of-domain datasets. 

In this paper, we propose a novel hybrid Mamba and MHA model (MambAttention) for generalizable single-channel speech enhancement. MambAttention comprises both time- and frequency-Mamba and MHA modules. \Change{As opposed to \cite{lenz2025jamba, rensamba, fathullah23_interspeech}, the time- and frequency-MHA modules in our MambAttention model are placed before their respective time- and frequency-Mamba blocks. Additionally, in contrast to DeFT-Mamba \cite{deftmamba}, our MambAttention model - developed independently - processes the encoded input along the time-dimension before the frequency-dimension. As we will demonstrate, this ordering yields superior in- and out-of-domain speech enhancement performance. Moreover, while DeFT-Mamba employs a GCB to shift features by one frequency bin or one time frame before applying the MHA and Mamba blocks to process across frequency or time, our model does not use a GCB.} \Change{More importantly, our MambAttention model shares weights between the MHA modules within each layer, which sets it apart from most existing hybrid attention models \cite{pandey2022self,lenz2025jamba,rensamba, fathullah23_interspeech, sui2024tramba, deftmamba}.} By sharing the weights between the MHA modules in each layer, our MambAttention model jointly attends to both time and frequency features. We find that this substantially improves generalization across speakers and noise types. To the best of our knowledge, MambAttention is the first model to combine Mamba with MHA across time and frequency for speech enhancement.

While \textit{VoiceBank+Demand} \cite{voicebank,demand} is a widely-used benchmark for single-channel speech enhancement, the test set contains neither babble noise nor speech-shaped noise (SSN) and the signal-to-noise ratios (SNRs) of both training and test files are not lower than \SI{0}{dB}. This means speech enhancement systems trained and tested only on \textit{VoiceBank+Demand} are neither exposed to nor evaluated in difficult listening conditions. Motivated by this, we propose a new benchmark: \textit{VoiceBank+Demand Extended} (\textit{VB-DemandEx}). Compared to the \textit{VoiceBank+Demand} dataset, our \textit{VB-DemandEx} comprises much lower signal-to-noise ratios and a larger variety of noise types. To evaluate the performance of MambAttention, we train our models on the \textit{VB-DemandEx} training set, and test on the in-domain \textit{VB-DemandEx} test set as well as two out-of-domain test sets from \textit{DNS 2020} \cite{reddy20_interspeech} and \textit{EARS-WHAM\_v2} \cite{richter24_interspeech}. Results show that our MambAttention model significantly outperforms existing state-of-the-art LSTM-, xLSTM-, Mamba-, and Conformer-based systems on the out-of-domain test sets across all reported evaluation metrics, while still delivering state-of-the-art performance on \Change{the} in-domain test set. Ablation studies on our proposed MambAttention model shows that the weight sharing mechanism positively impacts generalization performance. Additionally, we find that placing the MHA modules before the Mamba blocks significantly improves generalization performance.
% In all cases, our MambAttention model matches the in-domain enhancement performance of the state-of-the-art baselines.
Furthermore, we find that augmenting existing LSTM-, and xLSTM-based speech enhancement systems with our proposed MHA modules also greatly improves generalization performance; however, our MambAttention model remains superior across all datasets and reported evaluation metrics. 

To gain further insights, we visualize the latent features of our MambAttention model, and the LSTM-, xLSTM-, Mamba-, and Conformer-based models. This reveals that after being processed by our MambAttention model and the attention-based Conformer model, the in-domain and out-of-domain samples appear much closer to each other compared to the attention-free LSTM, xLSTM, and Mamba models. This suggests that MHA encourages the model to learn dataset-invariant representations. 
% This observation aligns with the superior generalization performance of these attention-based models compared to LSTM, xLSTM, and Mamba.
Finally, our MambAttention model shows superior scalability with respect to dataset size when trained on the large-scale \textit{DNS 2020} dataset, as it outperforms the LSTM, xLSTM, Mamba, and Conformer baselines across all reported metrics.
Our major contributions are summarized as follows:
\begin{itemize}
    \item We propose a novel state-of-the-art hybrid MambAttention model combining Mamba and MHA for generalizable single-channel speech enhancement.
    \item We propose the \textit{VB-DemandEx} benchmark, which is inspired by \textit{VoiceBank+Demand}, but features substantially lower SNRs and more noise types.
    \item We demonstrate that weight sharing between time- and frequency-MHA modules in our MambAttention model contributes to its state-of-art generalization performance.
    \item We show that combining our shared time- and frequency-MHA modules with LSTM- and xLSTM-based models significantly improves their generalization performance.
\end{itemize}
% The rest of the paper is organized as follows. In \autoref{sec:method}, we describe the building blocks of our MambAttention model. \autoref{sec:experiments} details the datasets used, presents a model overview, and the experimental details as well as the evaluation metrics used. Results are presented in \autoref{sec:results}, and limitations of the model are discussed in \autoref{sec:discussion}. Concluding remarks are given in \autoref{sec:conclusion}.
Code, audio samples, model weights, and the proposed dataset are publicly available.\footnote{\url{https://github.com/NikolaiKyhne/MambAttention}}


==> Text/Jan_Oestergaard_biography.tex <==
\begin{IEEEbiography}[{\includegraphics
[width=1in,height=1.25in,clip,
keepaspectratio]{Pix/Biography/Jan_Oestergaard_image.jpg}}]
{Jan Østergaard} (Senior Member, IEEE) received the M.Sc. degree from Aalborg University, Aalborg, Denmark, in 1999 and the PhD degree (with cum laude) from Delft University of Technology, Delft, The Netherlands, in 2007. From 1999 to 2002, he worked as an R\&D Engineer at ETI A/S, Aalborg, and from 2002 to 2003, he was an R\&D Engineer with ETI Inc., VA, USA. Between September 2007 and June 2008, he was a Postdoctoral Researcher at The University of Newcastle, NSW, Australia. Dr. Østergaard is currently a Full Professor in Information Theory and Signal Processing, Head of the Section on AI and Sound, and Head of the Centre on Acoustic Signal Processing Research (CASPR), at Aalborg University. He has received a Danish Independent Research Council’s Young Researcher’s Award, a Best PhD Thesis award by the European Association for Signal Processing (EURASIP), and fellowships from the Danish Independent Research Council, the Villum Foundations Young Investigator Programme, and the Novo Nordic Foundations. He is an Associate Editor for the IEEE Transactions on Information Theory. His research interests are in the areas of statistical signal processing, information theory, and acoustic signal processing.
\end{IEEEbiography}

% \begin{IEEEbiographynophoto}
% {Jan Østergaard} (Senior Member, IEEE) received the M.Sc. degree from Aalborg University, Aalborg, Denmark, in 1999 and the PhD degree (with cum laude) from Delft University of Technology, Delft, The Netherlands, in 2007. From 1999 to 2002, he worked as an R\&D Engineer at ETI A/S, Aalborg, and from 2002 to 2003, he was an R\&D Engineer with ETI Inc., VA, USA. Between September 2007 and June 2008, he was a Postdoctoral Researcher at The University of Newcastle, NSW, Australia. Dr. Østergaard is currently a Full Professor in Information Theory and Signal Processing, Head of the Section on AI and Sound, and Head of the Centre on Acoustic Signal Processing Research (CASPR), at Aalborg University. He has received a Danish Independent Research Council’s Young Researcher’s Award, a Best PhD Thesis award by the European Association for Signal Processing (EURASIP), and fellowships from the Danish Independent Research Council, the Villum Foundations Young Investigator Programme, and the Novo Nordic Foundations. He is an Associate Editor for the IEEE Transactions on Information Theory. His research interests are in the areas of statistical signal processing, information theory, and acoustic signal processing.
% \end{IEEEbiographynophoto}

==> Text/Jesper_Jensen_biography.tex <==
\begin{IEEEbiography}[{\includegraphics
[width=1in,height=1.25in,clip,
keepaspectratio]{Pix/Biography/Jesper_Jensen_image.jpg}}]
{Jesper Jensen} (Member, IEEE) received the M.Sc. degree in electrical
engineering and the Ph.D. degree in signal processing
from Aalborg University, Aalborg, Denmark,
in 1996 and 2000, respectively. From 1996 to 2000,
he was with the Center for Person Kommunikation
(CPK), Aalborg University, as a Ph.D. student and
Assistant Research Professor. From 2000 to 2007, he
was a Post-Doctoral Researcher and Assistant Professor
with Delft University of Technology, Delft,
The Netherlands, and an External Associate Professor
with Aalborg University. Currently, he is a Fellow of Oticon, Denmark,  
where he is responsible for research and development of signal processing and machine learning concepts
for hearing aid applications. He is a Professor with the Section for AI and Sound (AIS), Department of Electronic Systems, at
Aalborg University. He is also a co-founder of the Centre for Acoustic Signal
Processing Research (CASPR) at Aalborg University. His main interests are
in the area of acoustic signal processing, including signal retrieval from
noisy observations, coding, speech and audio modification and synthesis,
intelligibility enhancement of speech signals, signal processing for hearing
aid applications, and perceptual aspects of signal processing.
\end{IEEEbiography}

% \begin{IEEEbiographynophoto}
% {Jesper Jensen} (Member, IEEE) received the M.Sc. degree in electrical
% engineering and the Ph.D. degree in signal processing
% from Aalborg University, Aalborg, Denmark,
% in 1996 and 2000, respectively. From 1996 to 2000,
% he was with the Center for Person Kommunikation
% (CPK), Aalborg University, as a Ph.D. student and
% Assistant Research Professor. From 2000 to 2007, he
% was a Post-Doctoral Researcher and Assistant Professor
% with Delft University of Technology, Delft,
% The Netherlands, and an External Associate Professor
% with Aalborg University. Currently, he is a Fellow of Oticon, Denmark,  
% where he is responsible for research and development of signal processing and machine learning concepts
% for hearing aid applications. He is a Professor with the Section for AI and Sound (AIS), Department of Electronic Systems, at
% Aalborg University. He is also a co-founder of the Centre for Acoustic Signal
% Processing Research (CASPR) at Aalborg University. His main interests are
% in the area of acoustic signal processing, including signal retrieval from
% noisy observations, coding, speech and audio modification and synthesis,
% intelligibility enhancement of speech signals, signal processing for hearing
% aid applications, and perceptual aspects of signal processing.
% \end{IEEEbiographynophoto}

==> Text/Nikolai_Kuehne_biography.tex <==
\begin{IEEEbiography}[{\includegraphics
[width=1in,height=1.25in,clip,
keepaspectratio]{Pix/Biography/Nikolai_Kuehne_image.jpg}}]
{Nikolai Lund Kühne}
(Graduate Student Member, IEEE) received the B.Sc. degree in Mathematical Engineering from Aalborg University, Aalborg, Denmark, in 2023. Since 2024, he has been working on a joint long master's thesis and Ph.D at the Centre for Acoustic Signal Processing Research (CASPR) and the Department of Electronic Systems, Aalborg University. His research interests include sequence modelling neural networks, speech large language models, and single-channel speech enhancement.
\end{IEEEbiography}

% \begin{IEEEbiographynophoto}
% {Nikolai Lund Kühne}
% (Graduate Student Member, IEEE) received the B.Sc. degree in Mathematical Engineering from Aalborg University, Aalborg, Denmark, in 2023. Since 2024, he has been working on a joint long master's thesis and Ph.D at the Centre for Acoustic Signal Processing Research (CASPR) and the Department of Electronic Systems, Aalborg University. His research interests include sequence modelling neural networks, speech large language models, and single-channel speech enhancement.
% \end{IEEEbiographynophoto}

==> Text/Zheng-Hua_Tan_biography.tex <==
\begin{IEEEbiography}[{\includegraphics
[width=1in,height=1.25in,clip,
keepaspectratio]{Pix/Biography/Zheng-Hua_Tan_image.jpg}}]
{Zheng-Hua Tan} (Senior Member, IEEE) received the B.Sc. and M.Sc. degrees in electrical engineering from Hunan University, Changsha, China, in 1990 and 1996, respectively, and the Ph.D. degree in electronic engineering from Shanghai Jiao Tong University (SJTU), Shanghai, China, in 1999. He is currently a Professor with the Department of Electronic Systems and a Co-Head of the Centre for Acoustic Signal Processing Research, Aalborg University, Aalborg, Denmark. He is also a Co-Lead of the Pioneer Centre for AI, Denmark. He was a Visiting Scientist with the Computer Science and Artificial Intelligence Laboratory, MIT, Cambridge, MA, USA, an Associate Professor with the Department of Electronic Engineering, SJTU, Shanghai, China, and a Postdoctoral Fellow with AI Laboratory, KAIST, Daejeon, Korea. His research interests include machine learning, deep learning, noise-robust speech processing, and multimodal signal processing. He has (co-)authored over 280 peer-reviewed papers. His works have been recognized by the IEEE Signal Processing Society 2022 Best Paper Award and International Speech Communication Association 2022 Best Research Paper Award. He is the Lead Editor for IEEE Journal of Selected Topics in Signal Processing Special Series on AI in Signal and Data Science. He served as the elected Chair of IEEE SPS Machine Learning for Signal Processing Technical Committee, a Member of IEEE SPS Technical Directions Board and Conferences Board, an Associate Editor for the IEEE TRANSACTIONS ON AUDIO, SPEECH AND LANGUAGE PROCESSING. He is the General Chair for ICASSP 2029 and a TPC Co-Chair for ICASSP 2028. He was a TPC Vice-Chair for ICASSP 2024 and the General Chair for IEEE MLSP 2018.
\end{IEEEbiography}


% \begin{IEEEbiographynophoto}
% {Zheng-Hua Tan} (Senior Member, IEEE) received the B.Sc. and M.Sc. degrees in electrical engineering from Hunan University, Changsha, China, in 1990 and 1996, respectively, and the Ph.D. degree in electronic engineering from Shanghai Jiao Tong University (SJTU), Shanghai, China, in 1999. He is currently a Professor with the Department of Electronic Systems and a Co-Head of the Centre for Acoustic Signal Processing Research, Aalborg University, Aalborg, Denmark. He is also a Co-Lead of the Pioneer Centre for AI, Denmark. He was a Visiting Scientist with the Computer Science and Artificial Intelligence Laboratory, MIT, Cambridge, MA, USA, an Associate Professor with the Department of Electronic Engineering, SJTU, Shanghai, China, and a Postdoctoral Fellow with AI Laboratory, KAIST, Daejeon, Korea. His research interests include machine learning, deep learning, noise-robust speech processing, and multimodal signal processing. He has (co-)authored over 280 peer-reviewed papers. His works have been recognized by the IEEE Signal Processing Society 2022 Best Paper Award and International Speech Communication Association 2022 Best Research Paper Award. He is the Lead Editor for IEEE Journal of Selected Topics in Signal Processing Special Series on AI in Signal and Data Science. He served as the elected Chair of IEEE SPS Machine Learning for Signal Processing Technical Committee, a Member of IEEE SPS Technical Directions Board and Conferences Board, an Associate Editor for the IEEE TRANSACTIONS ON AUDIO, SPEECH AND LANGUAGE PROCESSING. He is the General Chair for ICASSP 2029 and a TPC Co-Chair for ICASSP 2028. He was a TPC Vice-Chair for ICASSP 2024 and the General Chair for IEEE MLSP 2018.
% \end{IEEEbiographynophoto}
